Bidding in Multi-Unit Auctions under Limited Information

We study multi-unit auctions in which bidders have limited knowledge of opponent strategies and values. We characterize optimal prior-free bids; these bids minimize the maximal loss in expected utility resulting from uncertainty surrounding opponent behavior. Optimal bids are readily computable despite bidders having multi-dimensional private information, and in certain cases admit closed-form solutions. In the pay-as-bid auction the minimax-loss bid is unique; in the uniform-price auction the minimax-loss bid is unique if the bidder is allowed to determine the quantities for which they bid, as in many practical applications. We compare minimax-loss bids and auction outcomes across auction formats, and derive testable predictions.

==> tikz-loss-pab.tex <==
1.0000	50.0000
2.0000	44.4444
3.0000	42.1875
4.0000	40.9600
5.0000	40.1878
6.0000	39.6569
7.0000	39.2696
8.0000	38.9744
9.0000	38.7420
10.0000	38.5543
11.0000	38.3995
12.0000	38.2697
13.0000	38.1592
14.0000	38.0640
15.0000	37.9812
16.0000	37.9085
17.0000	37.8442
18.0000	37.7868
19.0000	37.7354
20.0000	37.6889
21.0000	37.6469
22.0000	37.6085
23.0000	37.5735
24.0000	37.5413
25.0000	37.5117


==> tikz-loss-upa.tex <==
1.0000	38.1966
2.0000	30.7979
3.0000	28.3119
4.0000	27.1554
5.0000	26.5188
6.0000	26.1295
7.0000	25.8736
8.0000	25.6961
9.0000	25.5680
10.0000	25.4723
11.0000	25.3990
12.0000	25.3415
13.0000	25.2957
14.0000	25.2585
15.0000	25.2280
16.0000	25.2025
17.0000	25.1811
18.0000	25.1629
19.0000	25.1474
20.0000	25.1339
21.0000	25.1222
22.0000	25.1120
23.0000	25.1030
24.0000	25.0951
25.0000	25.0880


==> tikz-points-rev-pab-mean-n10.tex <==
1.0000	84.9570
2.0000	87.8334
3.0000	87.1812
4.0000	86.8773
5.0000	86.6818
6.0000	86.5226
7.0000	86.3972
8.0000	86.3062
9.0000	86.2286
10.0000	86.1656


==> tikz-points-rev-pab-mean-n2.tex <==
1.0000	61.6159
2.0000	58.2855
3.0000	57.1332
4.0000	56.5685
5.0000	56.1809
6.0000	55.9186
7.0000	55.7189
8.0000	55.5718
9.0000	55.4518
10.0000	55.3594


==> tikz-points-rev-pab-mean-n5.tex <==
1.0000	75.8830
2.0000	75.7450
3.0000	74.8903
4.0000	74.4251
5.0000	74.1334
6.0000	73.9202
7.0000	73.7602
8.0000	73.6400
9.0000	73.5443
10.0000	73.4647


==> tikz-points-rev-upa-mean-n10.tex <==
1.0000	90.3109
2.0000	89.3759
3.0000	92.1703
4.0000	93.4601
5.0000	94.1863
6.0000	94.6375
7.0000	94.9179
8.0000	95.1169
9.0000	95.2667
10.0000	95.3811


==> tikz-points-rev-upa-mean-n2.tex <==
1.0000	48.4823
2.0000	47.3918
3.0000	47.3530
4.0000	47.2202
5.0000	47.1841
6.0000	47.1659
7.0000	47.1345
8.0000	47.1210
9.0000	47.1146
10.0000	47.1022


==> tikz-points-rev-upa-mean-n5.tex <==
1.0000	73.6833
2.0000	71.3791
3.0000	72.5897
4.0000	73.2003
5.0000	73.5761
6.0000	73.8136
7.0000	73.9643
8.0000	74.0617
9.0000	74.1375
10.0000	74.2046


==> tikz-points-upa-rev-higher-n10.tex <==
1.0000	72.6000
2.0000	54.0000
3.0000	67.1000
4.0000	72.8000
5.0000	75.1000
6.0000	76.9000
7.0000	78.1000
8.0000	78.6000
9.0000	79.3000
10.0000	79.9000


==> tikz-points-upa-rev-higher-n2.tex <==
1.0000	29.1400
2.0000	0.0000
3.0000	0.5000
4.0000	0.0000
5.0000	0.0000
6.0000	0.0000
7.0000	0.0000
8.0000	0.0000
9.0000	0.0000
10.0000	0.0000


==> tikz-points-upa-rev-higher-n5.tex <==
1.0000	53.4500
2.0000	26.7000
3.0000	37.4000
4.0000	41.4500
5.0000	43.8000
6.0000	45.4000
7.0000	46.2000
8.0000	46.9500
9.0000	47.4500
10.0000	47.8000

